An Ancient Brown Dwarf Transiting a Metal-Poor Thick Disk Star

We report the discovery of TOI-7019b, the first transiting brown dwarf (BD) known to orbit a star that is part of the Milky Way's ancient thick disk, as defined chemically ([Fe/H] $= -0.79 \pm 0.05$ dex, [$\alpha$/Fe] $= +0.26 \pm 0.05$ dex, [M/H] $= -0.59 \pm 0.06$ dex) and kinematically ($v_{\perp} \approx 150 \pm 1$ km s$^{-1}$). We estimate a system age $\tau = 12 \pm 2$ Gyr by fitting the host star's spectrum and spectral energy distribution to alpha-enhanced isochrones, and independently using the age-metallicity relation of the thick disk. This makes TOI-7019 by far the most metal-poor and ancient BD host known to date. We measure a BD mass of $61.3 \pm 2.1$ $M_{\rm J}$ and radius of $0.82 \pm 0.02$ $R_{\rm J}$ from a joint analysis of transit photometry and radial velocity measurements, along with an orbital period of $48.2592 \pm 0.0001$ days and an orbital eccentricity of $0.403 \pm 0.002$. The measured radius appears $12.3\% \pm 2.8\%$ larger than predicted relative to standard evolutionary models for old, metal-poor brown dwarfs, hinting at missing physics like the magnetic inhibition of convection. TOI-7019b lowers the probed metallicity regime for transiting BDs by over a factor of two, making it a benchmark system to test evolutionary models in the low-metallicity regime. Future measurements of TOI-7019b's atmosphere will test whether a brown dwarf's atmospheric composition tracks its host star's abundances, as expected for binary-like co-formation.

==> toi7019_rvs_stub.tex <==
2460780.954943 & 7077.9 & 47.0 \\
2460792.882175 & 8329.5 & 29.1 \\
2460798.880485 & 7840.6 & 44.0 \\
2460803.816594 & 6922.7 & 43.0 \\
2460810.805074 & 4060.3 & 53.5%
